Data driven reconstruction using frames and Riesz bases

We study the problem of regularization of inverse problems adopting a purely data driven approach, by using the similarity to the method of regularization by projection. We provide an application of a projection algorithm, utilized and applied in frames theory, as a data driven reconstruction procedure in inverse problems, generalizing the algorithm proposed by the authors in Inverse Problems 36 (2020), n. 12, 125009, based on an orthonormalization procedure for the training pairs. We show some numerical experiments, comparing the different methods.

==> introduction.tex <==
\section{Introduction}\label{sec:intro}
Inverse problems are concerned with the reconstruction of an unknown quantity $u \in \U$ from its indirect measurements $y \in \Y$ which are related by the \emph{forward model} $T \colon \U \to \Y$ that describes the relationship between the quantities of interest and the measurements. 
The forward operator $T$ models the physics of data acquisition and may involve, for instance, integral transforms (such as the Radon transform, see for instance \cite{Nat01,NatWue01,Kuc13}) and partial differential equations (PDEs) (see for instance~\cite{Isa90,Sym09}). 

Previously inverse problems were considered \emph{model driven}, meaning that the physics and chemistry of the acquisition process were expressed as accurately as possible with mathematical formulas. Typically this allows to write the inverse problem as an operator equation
\begin{equation}\label{eq:Au=y}
Tu=y\;.
\end{equation}
With the rise of the area of big data, \emph{data driven} approaches (that means \emph{avoiding} modeling of the operator $T$) have emerged (see \cite{ArrMaaOktScho19}). They are attractive because they do not require the forward operator explicitly, and often yield superior visual quality of the reconstruction. Instead these approaches require a series of training data.

Currently there is no adequate theory for purely data driven regularisation 
in inverse problems, i.e. a theory in the setting when the forward operator is given only via \emph{training pairs} 
\begin{equation}\label{eq:pairs}
\{\ui, \yi \} \quad \text{such that} \quad T\ui= \yi.
\end{equation}
In \cite{AspKorSch20} we made a first step of an analysis for purely data driven regularization by utilizing the similarity to the concept of \emph{regularization by projection}.
We demonstrated that regularisation by projection~\cite{Sei80,EngHanNeu96} and variational regularisation~\cite{SchGraGroHalLen09} can be formulated in a data driven setting and usual results such as convergence and stability can be obtained. 

As mentioned above the proposed method in \cite{AspKorSch20} does not require the 
explicit knowledge of the operator $T$ but only information on training pairs, 
which need to be normalized. For practical applications and in theoretical considerations 
the training pairs need to be orthonormalized, which we implemented via Gram-Schmidt. 
This paper checks alternatives to the orthonormalization procedure, such as \commentO{Leon, was genau rein QR, $L^*L$, decomposition}. In particular we investigate frame decompositions, which 
allow a generalization of the theory of \cite{AspKorSch20} to \emph{Riesz frames}. One of the motivations for studying frames came from the practical need to reconstruct the solution of \autoref{eq:Au=y} from \emph{redundant} training data. So far all existing methods based on projection need to filter out redundant data in a preprocessing step.

The paper is organised as follows. In \autoref{sec:GS} we review basic results from \cite{AspKorSch20}. In \autoref{sec:frames} we review basic facts on \emph{frames} and \emph{Riesz bases}, which are applied in \autoref{sec:dd} to data driven regularization. Finally we present 
numerical results in \autoref{sec:num} \commentO{etc...}


==> reg_proj.tex <==
\section{Gram-Schmidt orthogonalization as in \cite{AspKorSch20}} \label{sec:GS}
\emph{Regularization by projection} consists in approximating the solution $u^\dagger$ of \autoref{eq:Au=y} by the \emph{minimum norm solution} of the projected equation
\begin{equation} \label{TP_n u = y}
TP_n u = y.
\end{equation}
The minimum norm solution of this equation is unique and is given by
\begin{equation}
\udn = (TP_n)^\dagger y,
\end{equation}
where $(TP_n)^\dagger$ denotes the Moore-Penrose inverse of $TP_n$ (see \cite{Nas76}). The projection takes place in the image space $\U$, hence the superscript in our notation $\udn$.

\begin{center}
The topic of \cite{AspKorSch20} was to find $\udn$ by making use of the training data \autoref{eq:pairs} without explicit knowledge of the operator $T$.
\end{center}

This was numerically realized as follows: 
\begin{enumerate}
\item Application of the Gram-Schmidt orthogonalisation to the training data 
      $\set{y^i: i=1,\ldots,n}$ gives an orthonormal basis 
      $\set{\underline{y}^i: i=1,\ldots,n}$ of $\Y_n$.
\item Then $T {\underline u}^i=\underline{y}^i$ is solved. This can in fact realized with 
      the formula:
	  \begin{equation}\label{bu^k_expr1}
	     {\underline u}^i = \frac{u^i - \mysum{k}{1}{i-1} (y^i, \underline{y}^k) 
                            {\underline u}^k}{\norm{y^i- P_{{\mathcal Y}_{i-1}}y^i}} 
	     \quad \forall i \in \N.
	  \end{equation} 
\item Finally we get 
      \begin{equation} \label{eq:udn2}
	    \udn = T^{-1} P_{{\mathcal Y}_n} y = \mysum{i}{1}{n} \inner{y}{{\underline y}^i}{\underline u}^i.
	\end{equation}
\end{enumerate}
The main result of \cite{AspKorSch20} is a weak convergence result, which holds under the 
following assumption: 
\begin{assumption}\label{ass:l1_coefs_gt}
Let $\trimhat$ be an orthonormal basis obtained from the training images $\trim$ and denote 
$T \overline{u}^i=\overline{y}^i$ for all $i=1,2,\ldots$.
We assume that 
\begin{enumerate}
\item $\sum_{i=1}^\infty \abs{(u^\dagger, \orthim u^i)} < \infty.$
\item For every $n \in \N$ and any $i \geq n+1$ consider the following expansion 
%of $P_{\Y_n} \orthim y^i \in \Y_n$
%\begin{equation}\label{eq:qn}
$P_{\Y_n} \orthim y^i = \sum_{j=1}^n \beta_j^{i,n} \orthim y^j.$
%\end{equation}
We assume that there exists some $C > 0$ such that for every $n \in \N$ and every $i \geq n+1$, 
%\begin{equation}\label{eq:assump4}
$\sum_{j=1}^n (\beta_j^{i,n})^2 \leq C$.
% \textrm{ for every } i \geq n+1.
%\end{equation}
%where $C>0$ is a constant independent of $i$ and $n$. 
\end{enumerate}
\end{assumption}



\begin{theorem}[Theorems 9 and 11 in \cite{AspKorSch20}] \label{thm:engl_weak}
Let $y \in \range{T}$ be the exact right-hand side in~\autoref{eq:Au=y} and $\trpairs$ the training pairs defined in~\autoref{eq:pairs}. Let \autoref{ass:l1_coefs_gt} hold, then $\udn$ converges weakly to $u^\dagger$. 
\end{theorem}

 

%	
%where in the last inequality Assumption \ref{ass_l1} has been applied. Therefore, since the sequence $\{\udn\}$ is uniformly bounded, it contains a weakly convergent subsequence (that we don't relabel) such that
%	$\udn \weakto u$.
%	Since $A$ is bounded we get 
%	$A\udn \weakto Au.$
%	On the other hand, applying $A$ to~\autoref{u_n_inf_dim}, we get that
%	\begin{equation*}
%	A\udn = \mysum{i}{1}{n} (y, \underline{y}^i) \underline{y}^i \to y \quad \text{as $n \to \infty$},
%	\end{equation*}
%	hence $Au = y$ and since $A$ is injective this proves the assertion.
%\end{proof}

